Graduated Optimization of Black-Box Functions

Motivated by the problem of tuning hyperparameters in machine learning, we present a new approach for gradually and adaptively optimizing an unknown function using estimated gradients. We validate the empirical performance of the proposed idea on both low and high dimensional problems. The experimental results demonstrate the advantages of our approach for tuning high dimensional hyperparameters in machine learning.

==> sections/result_table_remain.tex <==
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c}
90\% Target & \textbf{SphereHighDim} & \textbf{BraninHoo} & \textbf{Himmelblau} & \textbf{Styblinski} & \textbf{LevyN13} & \textbf{MishraN2} & \textbf{GriewankN4}\\
\hline
AdaLipoTR & $\textbf{106.1}(\pm 21)$ & $21.24(\pm 34)$ & $14.58(\pm 6)$ & $30.6(\pm 20)$ & $\textbf{1.0}(\pm 0)$ & $5.74(\pm 2)$ & $10.51(\pm 2)$\\
AdaLipo & $995.31(\pm 47)$ & $21.91(\pm 27)$ & $19.52(\pm 12)$ & $49.9(\pm 27)$ & $\textbf{1.0}(\pm 0)$ & $\textbf{5.03}(\pm 2)$ & $21.69(\pm 7)$\\
PureRandomSearch & $1000.0(\pm 0)$ & $782.72(\pm 323)$ & $15.63(\pm 13)$ & $79.73(\pm 84)$ & $5.22(\pm 5)$ & $9.01(\pm 10)$ & $113.86(\pm 116)$\\
HierarchicalOptimisticOptimization & $1000.0(\pm 0)$ & $1000.0(\pm 0)$ & $\textbf{3.52}(\pm 0)$ & $\textbf{3.5}(\pm 0)$ & $\textbf{1.0}(\pm 0)$ & $5.51(\pm 0)$ & $\textbf{7.53}(\pm 0)$\\
GradOpt & $956.67(\pm 82)$ & $\textbf{21.23}(\pm 17)$ & $72.45(\pm 75)$ & $225.34(\pm 247)$ & $\textbf{1.0}(\pm 0)$ & $7.53(\pm 6)$ & $148.79(\pm 75)$\\
\hline
\end{tabular}
\end{adjustbox}
\\\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c}
95\% Target & \textbf{SphereHighDim} & \textbf{BraninHoo} & \textbf{Himmelblau} & \textbf{Styblinski} & \textbf{LevyN13} & \textbf{MishraN2} & \textbf{GriewankN4}\\
\hline
AdaLipoTR & $\textbf{155.08}(\pm 45)$ & $\textbf{21.8}(\pm 34)$ & $\textbf{18.73}(\pm 6)$ & $\textbf{32.71}(\pm 20)$ & $\textbf{1.0}(\pm 0)$ & $7.07(\pm 2)$ & $\textbf{11.72}(\pm 2)$\\
AdaLipo & $1000.0(\pm 0)$ & $25.54(\pm 27)$ & $27.03(\pm 18)$ & $64.8(\pm 40)$ & $\textbf{1.0}(\pm 0)$ & $\textbf{7.04}(\pm 2)$ & $30.22(\pm 14)$\\
PureRandomSearch & $1000.0(\pm 0)$ & $961.42(\pm 155)$ & $28.89(\pm 30)$ & $159.4(\pm 156)$ & $6.96(\pm 7)$ & $24.29(\pm 27)$ & $543.76(\pm 368)$\\
HierarchicalOptimisticOptimization & $1000.0(\pm 0)$ & $1000.0(\pm 0)$ & $21.31(\pm 6)$ & $232.67(\pm 384)$ & $\textbf{1.0}(\pm 0)$ & $9.47(\pm 0)$ & $13.47(\pm 0)$\\
GradOpt & $1000.0(\pm 0)$ & $22.22(\pm 19)$ & $213.15(\pm 156)$ & $324.61(\pm 271)$ & $\textbf{1.0}(\pm 0)$ & $13.36(\pm 10)$ & $308.24(\pm 97)$\\
\hline
\end{tabular}
\end{adjustbox}
\\\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c}
99\% Target & \textbf{SphereHighDim} & \textbf{BraninHoo} & \textbf{Himmelblau} & \textbf{Styblinski} & \textbf{LevyN13} & \textbf{MishraN2} & \textbf{GriewankN4}\\
\hline
AdaLipoTR & $\textbf{271.52}(\pm 55)$ & $\textbf{22.33}(\pm 34)$ & $\textbf{24.38}(\pm 7)$ & $\textbf{37.0}(\pm 19)$ & $\textbf{7.18}(\pm 2)$ & $\textbf{16.4}(\pm 15)$ & $\textbf{38.77}(\pm 97)$\\
AdaLipo & $1000.0(\pm 0)$ & $151.95(\pm 150)$ & $55.88(\pm 31)$ & $106.0(\pm 77)$ & $8.24(\pm 5)$ & $22.15(\pm 21)$ & $792.97(\pm 298)$\\
PureRandomSearch & $1000.0(\pm 0)$ & $1000.0(\pm 0)$ & $184.65(\pm 182)$ & $568.58(\pm 376)$ & $16.46(\pm 16)$ & $678.87(\pm 356)$ & $1000.0(\pm 0)$\\
HierarchicalOptimisticOptimization & $1000.0(\pm 0)$ & $1000.0(\pm 0)$ & $468.79(\pm 490)$ & $730.59(\pm 432)$ & $21.96(\pm 1)$ & $25.31(\pm 2)$ & $68.36(\pm 7)$\\
GradOpt & $1000.0(\pm 0)$ & $23.04(\pm 19)$ & $507.63(\pm 261)$ & $538.86(\pm 267)$ & $20.98(\pm 21)$ & $70.33(\pm 51)$ & $941.1(\pm 112)$\\
\hline
\end{tabular}
\end{adjustbox}
\\

==> sections/result_table_synt.tex <==
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c}
90\% Target & \textbf{HolderTable} & \textbf{Rosenbrock} & \textbf{Sphere} & \textbf{LinearSlope} & \textbf{DebN1}\\
\hline
PRS & $181.73(\pm 176)$ & $8.99(\pm 8)$ & $905.36(\pm 228)$ & $918.51(\pm 214)$ & $987.34(\pm 92)$\\
HOO & $56.48(\pm 10)$ & $7.6(\pm 1)$ & $952.47(\pm 49)$ & $32.96(\pm 2)$ & $\textbf{31.0}(\pm 0)$\\
AdaLipo & $49.34(\pm 31)$ & $\textbf{1.0}(\pm 0)$ & $49.59(\pm 15)$ & $11.11(\pm 5)$ & $961.54(\pm 148)$\\
AdaLipoTR & $\textbf{39.0}(\pm 32)$ & $\textbf{1.0}(\pm 0)$ & $\textbf{26.3}(\pm 4)$ & $\textbf{6.74}(\pm 1)$ & $147.29(\pm 152)$\\
GradOpt & $86.46(\pm 85)$ & $29.01(\pm 29)$ & $490.13(\pm 120)$ & $1000.0(\pm 0)$ & $965.39(\pm 146)$\\
\hline
\end{tabular}
\end{adjustbox}
\\\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c}
95\% Target & \textbf{HolderTable} & \textbf{Rosenbrock} & \textbf{Sphere} & \textbf{LinearSlope} & \textbf{DebN1}\\
\hline
PRS & $355.85(\pm 312)$ & $19.01(\pm 18)$ & $987.94(\pm 74)$ & $993.66(\pm 45)$ & $1000.0(\pm 0)$\\
HOO & $58.7(\pm 10)$ & $7.6(\pm 1)$ & $1000.0(\pm 0)$ & $47.61(\pm 3)$ & $\textbf{31.0}(\pm 0)$\\
AdaLipo & $79.57(\pm 45)$ & $\textbf{1.0}(\pm 0)$ & $94.55(\pm 40)$ & $36.05(\pm 22)$ & $995.88(\pm 29)$\\
AdaLipoTR & $\textbf{45.23}(\pm 32)$ & $\textbf{1.0}(\pm 0)$ & $\textbf{35.9}(\pm 7)$ & $\textbf{6.97}(\pm 0)$ & $156.82(\pm 151)$\\
GradOpt & $337.22(\pm 218)$ & $46.33(\pm 42)$ & $805.56(\pm 145)$ & $1000.0(\pm 0)$ & $992.92(\pm 70)$\\
\hline
\end{tabular}
\end{adjustbox}
\\\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c}
99\% Target & \textbf{HolderTable} & \textbf{Rosenbrock} & \textbf{Sphere} & \textbf{LinearSlope} & \textbf{DebN1}\\
\hline
PRS & $809.73(\pm 320)$ & $97.86(\pm 103)$ & $1000.0(\pm 0)$ & $1000.0(\pm 0)$ & $1000.0(\pm 0)$\\
HOO & $58.7(\pm 10)$ & $7.6(\pm 1)$ & $1000.0(\pm 0)$ & $152.15(\pm 9)$ & $\textbf{31.0}(\pm 0)$\\
AdaLipo & $137.38(\pm 52)$ & $\textbf{1.0}(\pm 0)$ & $979.69(\pm 94)$ & $960.99(\pm 153)$ & $1000.0(\pm 0)$\\
AdaLipoTR & $\textbf{50.4}(\pm 31)$ & $\textbf{1.0}(\pm 0)$ & $\textbf{59.24}(\pm 11)$ & $\textbf{7.04}(\pm 0)$ & $182.3(\pm 150)$\\
GradOpt & $671.45(\pm 281)$ & $130.77(\pm 108)$ & $999.06(\pm 9)$ & $1000.0(\pm 0)$ & $1000.0(\pm 0)$\\
\hline
\end{tabular}
\end{adjustbox}
\\
